Bounding Membership Inference

Differential Privacy (DP) is the de facto standard for reasoning about the privacy guarantees of a training algorithm. Despite the empirical observation that DP reduces the vulnerability of models to existing membership inference (MI) attacks, a theoretical underpinning as to why this is the case is largely missing in the literature. In practice, this means that models need to be trained with DP guarantees that greatly decrease their accuracy. In this paper, we provide a tighter bound on the positive accuracy (i.e., attack precision) of any MI adversary when a training algorithm provides $(\varepsilon, \delta)$-DP. Our bound informs the design of a novel privacy amplification scheme: an effective training set is sub-sampled from a larger set prior to the beginning of training. We find this greatly reduces the bound on MI positive accuracy. As a result, our scheme allows the use of looser DP guarantees to limit the success of any MI adversary; this ensures that the model's accuracy is less impacted by the privacy guarantee. While this clearly benefits entities working with far more data than they need to train on, it can also improve the accuracy-privacy trade-off on benchmarks studied in the academic literature. Consequently, we also find that subsampling decreases the effectiveness of a state-of-the-art MI attack (LiRA) much more effectively than training with stronger DP guarantees on MNIST and CIFAR10. We conclude by discussing implications of our MI bound on the field of machine unlearning.

==> Abstract.tex <==
\begin{abstract}
    Differential Privacy (DP) is the de facto standard for reasoning about the privacy guarantees of a training algorithm. Despite the empirical observation that DP reduces the vulnerability of models to existing membership inference (MI) attacks, a theoretical underpinning as to why this is the case is largely missing in the literature. In practice, this means that models need to be trained with DP guarantees that greatly decrease their accuracy. In this paper, we provide a tighter bound on the positive accuracy (\ie attack precision) of any MI adversary when a training algorithm provides $\epsilon$-DP or $(\epsilon, \delta)$-DP. Our bound informs the design of a novel privacy amplification scheme, where an effective training set is sub-sampled from a larger set prior to the beginning of training, to greatly reduce the bound on MI accuracy. As a result, our scheme enables DP users to employ looser DP guarantees when training their model to limit the success of any MI adversary; this ensures that the model's accuracy is less impacted by the privacy guarantee. Finally, we discuss implications of our MI bound on the field of machine unlearning.
\end{abstract}

==> Discussion.tex <==
\section{Discussion}
\label{sec:discussion}



\subsection{Our Bound is Tighter than Earlier Results}

We first compare our main technical result, the bound on a MI adversary's success, with the two key baselines we identified earlier~\citep{sablayrolles2019white,erlingsson2019we}, noting that \citet{sablayrolles2019white} made assumptions on the conditional weight distribution which we and \citet{erlingsson2019we} did not. The setting described in Section \ref{ssec:scenario} is equivalent to the MI experiment defined by \citet{yeom2018privacy} when $\mathbb{P}_{\mathbf{x}_i}(1) = 0.5 ~\forall \mathbf{x}_i \in \{\mathbf{x}_1,\cdots,\mathbf{x}_N\}$. That is, if the training dataset was constructed by sampling data points from a larger dataset by a coin flip, then when the adversary is given any data point from the larger dataset to test there is a $50\%$ chance it was in the training set or not. Furthermore, recall that when $\mathbb{P}_{\mathbf{x}^*}(1) = 0.5$, then Theorem~\ref{thm:MI_pos_acc} reduces to bounds on the overall accuracy of any MI attack $f$ (as the bounds on positive and negative accuracy are the same).
We can thus compare the upper-bound on MI accuracy that we achieved with the current tightest bounds given by \citet{erlingsson2019we} and \citet{sablayrolles2019white} for $\epsilon$-DP; we stated these bounds earlier in \Cref{ssec:Prev_bounds}, where for the latter bound we also set $\mathbb{P}_{\mathbf{x}^*}(1) = 0.5$. 

Our bound, and these two previous bounds, are depicted in~\Cref{fig:MI_bounds}, where we see our bound given in Theorem \ref{thm:MI_pos_acc} is always tighter than both of the previous bounds. In particular, we see that it is closer to the one introduced by \citet{sablayrolles2019white} for small $\epsilon$ and closer to the one defined by \citet{erlingsson2019we} for large $\epsilon$. Notably, for $\epsilon = 1$, we bound the accuracy of an MI attack by $73.1\%$ whereas~\citet{erlingsson2019we} bound it by $81.6\%$, and~\citet{sablayrolles2019white}  by $75\%$.
For $\epsilon = 2$, we bound MI accuracy by $88\%$ whereas \citet{erlingsson2019we} bound it by $95\%$ and \citet{sablayrolles2019white} by $100\%$. Do note our bound generalizes for when the sampling probability is not $0.5$; we compare our bound with \citet{sablayrolles2019white} in this setting in \Cref{fig:sab_MI_bound_prob}, though recall once again \citet{sablayrolles2019white} made assumptions on the weight distribution we did not.



\subsection{We can Bound Generalization Error}

\citet{yeom2018privacy} studied adversaries that took advantage of a generalization gap $R_g$ between training datapoints and non-training datapoints. In particular for Adversary 1 in \citet{yeom2018privacy}, they showed its MI accuracy is $(R_g/B +1)/2$ (Theorem 2 in \citet{yeom2018privacy}). That is, we have an adversary whose accuracy is completely determined by the generalization gap of the model. However, when training with $\epsilon$-DP the accuracy of all MI adversaries is bounded by our lower and upper-bound in Theorem \ref{thm:MI_pos_acc} (taking $\mathbb{P}_{\mathbf{x}^*}(1) = 0.5$ as we are looking at accuracy). Thus we have the following corollary.

\begin{corollary}[MI bounds Generalization Error]
For loss function upper-bounded by $B$ and $\epsilon$-DP training algorithm, we have $(1+e^{\epsilon})^{-1} \leq (R_g/B +1)/2 \leq (1+e^{-\epsilon})^{-1}$ where $R_g$ is the \textit{generalization gap} (Definition 3 in \citet{yeom2018privacy}, where their $D$ is our larger set, and their $S$ is the specific training set sampled from the larger set).
\end{corollary}

In particular this tells us how well the $\mathbb{P}_{\mathbf{x}^*}(1) = 0.5$ sampled dataset generalizes to having trained on the entire larger set. We believe this general procedure of using specific adversaries with accuracies dependent on values of interest (\eg the generalization gap here) and applying more general bounds to get a range for those values of interest is something future work can expand on.

\subsection{MI Accuracy vs. MI Advantage}

Previous work, particularly~\citet{yeom2018privacy} and~\citet{erlingsson2019we}, focused on membership advantage, which is essentially an improvement in accuracy of $f$ over the random guess of $50\%$ of drawing a point in the training dataset. %
More specifically, if we let $A(f)$ denote the accuracy of $f$, then membership advantage is computed as $2(A(f)-0.5)$.
We can generalize this to ask what the membership advantage of the positive accuracy of $f$ compared to the baseline $\mathbb{P}_{\mathbf{x}^*}(1)$ is for values other than only $0.5$.


Theorem \ref{thm:MI_pos_acc} gives us an upper bound on the positive accuracy and thus an upper bound on the positive advantage of $f$ denoted as $Ad(f)$: $Ad(f) = 2\left(A(f(\mathbf{x}^*,S) =1) - \mathbb{P}_{\mathbf{x}^*}(1)\right)
\leq 2 \left(\left({1+\frac{e^{-\epsilon}\mathbb{P}_{\mathbf{x}^*}(0)}{\mathbb{P}_{\mathbf{x}^*}(1)}}\right)^{-1} - \mathbb{P}_{\mathbf{x}^*}(1)\right)$. We plotted this advantage as a function of $\mathbb{P}_{\mathbf{x}^*}(1)$ for different fixed $\epsilon$ in Figure \ref{fig:MI_adv} (see Appendix~\ref{sec: Appendix B: Figures}). We observe that the advantage clearly depends on $\mathbb{P}_{\mathbf{x}^*}(1)$, and in fact for different $\epsilon$, the $\mathbb{P}_{\mathbf{x}^*}(1)$ resulting in the maximum advantage changes. In particular, $\mathbb{P}_{\mathbf{x}^*}(1) = 0.5$ is not close to the maximum advantage for large $\epsilon$, which shows how the fixed experiment proposed by \citet{yeom2018privacy} does not necessarily give the maximum advantage an adversary could have, whereas our result allows us to.




However, it should be noted that higher advantage here does not mean a higher upper bound on MI accuracy; as we already saw in \Cref{fig:MI_bound_prob}, the upper bound on accuracy increases monotonically with $\mathbb{P}_{\mathbf{x}^*}(1)$, in contrast to the bump observed with membership advantage.
This serves to differentiate the study of MI advantage and the study of MI accuracy for future work. 











==> Effect_of_Dataset_Sampling.tex <==
\section{The Amplification Effect of $\mathbb{P}_{\mathbf{x}^*}(1)$}
\label{sec: sampling_effect}


The above scenario is a specific instance of what Theorem \ref{thm:MI_pos_acc} implies. More generally, Theorem \ref{thm:MI_pos_acc} shows that decreasing $\mathbb{P}_{\mathbf{x}^*}(1)$ directly leads to a decrease in the upper bound of the accuracy an adversary has when predicting the presence of $x^*$ in the training dataset. %
That is, by simply reducing $\mathbb{P}_{\mathbf{x}^*}(1)$ an entity can reduce the accuracy of associating $\mathbf{x}^*$ to any specific set of models in a fashion similar to privacy amplification for DP, where low batch sampling probability increases privacy~\citep{beimel2010bounds,kasiviswanathan2011can,abadi2016deep}.


The importance of $\mathbb{P}_{\mathbf{x}^*}(1)$ against positive MI accuracy, defined as $\mathbb{P}(\mathbf{x}^*|S)$ where $S$ is any set of models, is depicted in~\Cref{fig:MI_bound_prob} (see Appendix~\ref{sec: Appendix B: Figures}), where for different $\epsilon$ we plotted the upper bound on positive accuracy given by Theorem \ref{thm:MI_pos_acc} as we change $\mathbb{P}_{\mathbf{x}^*}(1)$. In particular for $\epsilon=2$ when  $\mathbb{P}_{\mathbf{x}^*}(1) = 0.01$ (\ie $1\%$) we have the positive accuracy is bounded by $6.9\%$.




An interesting question is how does DP privacy amplification (which we get by sampling relatively small batches compared to the dataset) compare to the amplification we get from $\mathbb{P}_{\mathbf{x}^*}(0)/\mathbb{P}_{\mathbf{x}^*}(1)$ for our bound. Note that decreasing $\mathbb{P}_{\mathbf{x}^*}(0)/\mathbb{P}_{\mathbf{x}^*}(1)$ places no restriction on the sampling rate for batch sizes (which is how one would get DP privacy amplification) upto a point. After this point, the expectation of the training dataset size decreases and thus the lowest possible sampling rate $1/n$, where $n$ in the training set size, increases in expectation. Nevertheless, now including $q$ for DP privacy amplification, we can compare their effect by focusing on just the $e^{-q\epsilon_0}\mathbb{P}_{\mathbf{x}}(0)/\mathbb{P}_{\mathbf{x}}(1)$ term in the bound given by Theorem \ref{thm:MI_pos_acc}, where the goal is to maximize this in order the make the upper bound as small as possible. In particular, we see decreasing $q$ increases this term by $O(e^{-t})$ where as decreasing $\mathbb{P}_{\mathbf{x}^*}(1)$ increases this term by $O((1-t)/t)$, which is slower than $O(e^{-t})$ upto a point, then faster (do note that we are looking at the order as the variable $t$ decreases); Figure~\ref{fig:Priv_Amp_Comp} plots this relation. This same comparison holds more generally when comparing the effect of $\epsilon$ and $\mathbb{P}_{\mathbf{x}^*}(1)$.


More generally, what this says is that to defend against an adversary there needs to be some indistinguishability between models from adjacent datasets (the $\epsilon$-DP guarantee). However, after a certain point the uncertainty from sampling the training dataset is much more influential than the one obtained by making the models even less distinguishable. That said, one should note that sampling the training dataset may eventually significantly decrease the accuracy of models learned (from less data). This may put practical constraints on how much one can reduce $\mathbb{P}_{\mathbf{x}^*}(1)$. 




\begin{figure}[h]
    \centering
    \includegraphics[width=70mm]{imgs/Privacy_Amp_comparison.pdf}
    \caption{Comparing the DP amplification observed by decreasing batch probability (given by $e^{-t}$) to the amplification we observe from decreasing $\mathbb{P}_{\mathbf{x}}(1)$ (given by $(1-t)/t$)}
    \label{fig:Priv_Amp_Comp}
\end{figure}



==> Implications.tex <==
\anvith{@new section}
\section{Implication of MI Bounds}

Here we outline how MI 

==> consequences.tex <==
\section{Consequences}
\label{sec:consequences}

\subsection{Tighter Bound}

The setup described in Section \ref{ssec:scenario} is equivalent to the MI experiment defined by \cite{yeom2018privacy} when $\mathbb{P}_{\mathbf{x}_i}(1) = 0.5 ~\forall \mathbf{x}_i \in \{\mathbf{x}_1,\cdots,\mathbf{x}_N\}$. That is, if the training dataset was constructed by sampling data points from a larger dataset by a coin flip, then when the adversary is given any data point from the larger dataset to test there is a $50\%$ chance it was in the training set or not.%

Furthermore, recall that when $\mathbb{P}_{\mathbf{x}^*}(1) = 0.5$, then Theorem~\ref{thm:MI_pos_acc} reduces to bounds on the overall accuracy of any membership attack $f$ (as the bounds on positive and negative accuracy are the same).

We thus can compare the upper-bound on MI accuracy that we achieved with the current tightest bounds given by \cite{erlingsson2019we} and \cite{sablayrolles2019white} for $\epsilon$-DP; we stated these bounds earlier in \Cref{ssec:Prev_bounds}, where for the latter bound we also set $\mathbb{P}_{\mathbf{x}^*}(1) = 0.5$. Our bound, and these two previous bounds, are depicted in~\Cref{fig:MI_bounds}, where we see the bound given in Theorem \ref{thm:MI_pos_acc} is always tighter than both of the previous bounds. In particular, we see that it is closer to the one introduced by \citeauthor{sablayrolles2019white} bound for small $\epsilon$ and closer to the one defined by \citeauthor{erlingsson2019we} bound for large $\epsilon$.

Notably, for $\epsilon = 1$, we bound the accuracy of an MI attack by $73.1\%$ whereas~\citeauthor{erlingsson2019we} bound it by $81.6\%$, and~\citeauthor{sablayrolles2019white} bound it by $75\%$.
For $\epsilon = 2$, we bound the accuracy of an MI attack by $88\%$ whereas \citeauthor{erlingsson2019we} bound it by $95\%$ and \citeauthor{sablayrolles2019white} bound it by $100\%$.

\begin{figure}
    \centering
    \includegraphics[width=70mm]{imgs/more_MI_bounds.pdf}
    \caption{Comparing the upper bound to MI performance we achieved to that given by~\cite{erlingsson2019we} and~\cite{sablayrolles2019white}. In particular note we are tighter for all $\epsilon$.}
    \label{fig:MI_bounds}
\end{figure}


\subsection{The Effect of $\mathbb{P}_{\mathbf{x}^*}(1)$}


The above scenario is a specific instance of what Theorem \ref{thm:MI_pos_acc} implies. More generally, Theorem \ref{thm:MI_pos_acc} shows that decreasing $\mathbb{P}_{\mathbf{x}^*}(1)$ directly leads to a decrease in the upper bound of the accuracy an adversary has when predicting the presence of $x^*$ in the training dataset. %
That is, by simply reducing $\mathbb{P}_{\mathbf{x}^*}(1)$ an entity can reduce the accuracy of associating $\mathbf{x}^*$ to any specific set of models in a fashion similar to privacy amplification for DP \cite{balle2018improving} (where low batch sampling probability increases privacy).


The importance of $\mathbb{P}_{\mathbf{x}^*}(1)$ against positive MI accuracy, defined as $\mathbb{P}(\mathbf{x}^*|S)$ where $S$ is any set of models, is depicted in~\Cref{fig:MI_bound_prob}, where for different $\epsilon$ we plotted the upper bound on positive accuracy given by Theorem \ref{thm:MI_pos_acc} as we change $\mathbb{P}_{\mathbf{x}^*}(1)$. In particular for $\epsilon=2$ when  $\mathbb{P}_{\mathbf{x}^*}(1) = 0.01$ (\ie $1\%$) we have the positive accuracy is bounded by $6.9\%$.

\begin{figure}[h]
    \centering
    \includegraphics[width=70mm]{imgs/MI_bound_prob_many.pdf}
    \caption{Upper bound on MI positive accuracy as a function of $\mathbb{P}_{\mathbf{x}^*}(1)$}
    \label{fig:MI_bound_prob}
\end{figure}


An interesting question is how does DP privacy amplification (which we get by sampling relatively small batches compared to the dataset) compare to the amplification we get from $\mathbb{P}_{\mathbf{x}^*}(0)/\mathbb{P}_{\mathbf{x}^*}(1)$ for our bound. Note that decreasing $\mathbb{P}_{\mathbf{x}^*}(0)/\mathbb{P}_{\mathbf{x}^*}(1)$ places no restriction on the sampling rate for batch sizes (which is how one would get DP privacy amplification) upto a point (as the expectation of the training dataset size decreases and thus the lowest possible sampling rate $1/n$, where $n$ in the training set size, increases in expectation). Nevertheless, now including $q$ for DP privacy amplification, we can compare their effect by focusing on just the $e^{-q\epsilon_0}\mathbb{P}_{\mathbf{x}}(0)/\mathbb{P}_{\mathbf{x}}(1)$ term in the bound given by Theorem \ref{thm:MI_pos_acc}, where the goal is to maximize this in order the make the upper bound as small as possible. In particular, we see decreasing $q$ increases this term by $O(e^{-t})$ where as decreasing $\mathbb{P}_{\mathbf{x}^*}(1)$ increases this term by $O(1-t/t)$, which is slower than $O(e^{-t})$ upto a point, then faster (where note we are looking at the order as the variable $t$ decreases not increases); Figure~\ref{fig:Priv_Amp_Comp} plots this relation. This same comparison holds more generally when comparing the affect of $\epsilon$ and $\mathbb{P}_{\mathbf{x}^*}(1)$.


More generally, what this says is that to defend against an adversary there needs to be some indistinguishability between models from adjacent datasets (the $\epsilon$-DP guarantee). However, after a certain point the uncertainty from sampling the training dataset is much more influential than the one obtained by making the models even less distinguishable.




\begin{figure}[h]
    \centering
    \includegraphics[width=70mm]{imgs/Privacy_Amp_comparison.pdf}
    \caption{Comparing the DP amplification observed by decreasing batch probability (given by $e^{-t}$) to the amplification we observe from decreasing $\mathbb{P}_{\mathbf{x}}(1)$ (given by $\frac{1-t}{t}$)}
    \label{fig:Priv_Amp_Comp}
\end{figure}


\subsection{Importance to Data Deletion}
\label{ssec:data_deletion}

The ability for an entity to decrease the ability for an arbitrator to attribute a datapoint to a model also has consequences for machine unlearning and data deletion requests as mentioned in~\Cref{ssec:Unlearning}.


In particular if $\mathbb{P}(\mathbf{x}^* \in D|S)$ is sufficiently low, that is the likelihood of $S$ coming from $\mathbf{x}^*$ is low, then an entity could claim that they do not need to delete the users data since their model is most likely independent of that datapoint as it most likely came from a model without it: \ie leading to plausible deniability. This is similar to the logic presented by~\cite{sekhari2021remember} where unlearning is presented probablistically in terms of $(\epsilon,\delta)$-unlearning (which $(\epsilon,\delta)$-DP is sufficient for, but is not necessary).

We also observe an analogous result to~\cite{sekhari2021remember} where we can only handle a maximum number of deletion requests before no longer having sufficiently low probability. To be exact, let us say we do not need to undergo any unlearning process given a set of data deletion request $\hat{\mathbf{x}}^*$ if $\mathbb{P}(\hat{\mathbf{x}}^* \notin D|S) \geq B$ for some $B$ (\ie we are working with probability of not having that set of data in our training set which we want to be high). Note that we sampled data independently, thus if $\hat{\mathbf{x}}^* = \{\mathbf{x}_1^*,\mathbf{x}_2^*,\cdots,\mathbf{x}_m^*\}$, then $\mathbb{P}(\hat{\mathbf{x}}^* \notin D|S) = \mathbb{P}(\mathbf{x}_1^* \notin D|S) \cdots \mathbb{P}(\mathbf{x}_m^* \notin D|S)$.

Now, for simplicity, assume the probability of drawing all points into the datasets are the same, so that for all $\mathbf{x}_i^*$ we have the same bound given by Corollary \ref{cor:MI_neg_acc}, that is $\mathbb{P}(\mathbf{x}_i^* \notin D|S) > L$ for some $L \leq 1$. Then we have $\mathbb{P}(\hat{\mathbf{x}}^* \notin D|S) \geq L^m$ and so an entity does not need to unlearn if $L^m \geq B$, \ie if $m \leq \frac{\ln{1/B}}{\ln{1/L}} = \frac{\ln{B}}{\ln{L}}$. This gives a bound on how many deletion requests the entity can avoid in terms of the lower bound given in Corollary~\ref{cor:MI_neg_acc}.

In particular, note that if $\{\mathbf{x}_1 \cdots \mathbf{x}_N\}$ is the larger set of data points an entity is sampling from, and $\mathbb{P}_{\mathbf{x}}(1) = c/N$ $\forall \mathbf{x} \in \{\mathbf{x}_1 \cdots \mathbf{x}_N\}$, then the lower bound given by Corollary~\ref{cor:MI_neg_acc} is $\frac{1}{1+\frac{e^{-\epsilon}\frac{c}{N}}{1-\frac{c}{N}}}$. \cite{sekhari2021remember} showed that with typical DP the deletion requests grow linearly with the size of the training (in the above case $c$ represents the expected training set size). We thus compare a linear line w.r.t to $c$ to $\frac{\ln{B}}{\ln{L(c)}}$ (where $L$ is given in the earlier expression for the bound from Corollary~\ref{cor:MI_neg_acc}) in~\Cref{fig:} to observe their respective magnitude: we fix $B=0.8$,$N = 10000$ and $\epsilon = 1$ as we are interested in general trends. We observe that our deletion capacity is significantly higher for low expected training set sizes and is marginally lower than a linear trend for larger training set sizes.

\begin{figure}[h]
    \centering
    \includegraphics[width=70mm]{imgs/Deletion_capacity_vs_training_size.pdf}
    \caption{Comparing our deletion trend to the trend~\cite{sekhari2021remember} describes. In particular our number of deletions degrades with training size while theirs increasing.}
    \label{fig:}
\end{figure}



















==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

